Stability of Aggregation Graph Neural Networks

In this paper we study the stability properties of aggregation graph neural networks (Agg-GNNs) considering perturbations of the underlying graph. An Agg-GNN is a hybrid architecture where information is defined on the nodes of a graph, but it is processed block-wise by Euclidean CNNs on the nodes after several diffusions on the graph shift operator. We derive stability bounds for the mapping operator associated to a generic Agg-GNN, and we specify conditions under which such operators can be stable to deformations. We prove that the stability bounds are defined by the properties of the filters in the first layer of the CNN that acts on each node. Additionally, we show that there is a close relationship between the number of aggregations, the filter's selectivity, and the size of the stability constants. We also conclude that in Agg-GNNs the selectivity of the mapping operators is tied to the properties of the filters only in the first layer of the CNN stage. This shows a substantial difference with respect to the stability properties of selection GNNs, where the selectivity of the filters in all layers is constrained by their stability. We provide numerical evidence corroborating the results derived, testing the behavior of Agg-GNNs in real life application scenarios considering perturbations of different magnitude.

==> v13/sec_RTASM.tex <==
%!TEX root =../compiler_paper.tex


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\begin{figure}
% \centering\includegraphics[scale=0.8,angle=0]{../figures/fig7b.pdf}
% \caption{Schematic representation of the algebraic signal model}
% \label{fig_1}
%\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%

\subsection{Algebraic Signal Processing} \label{sec_alg_filters}%{Representation Theory of Algebras and Signal Models}

The convolution operation is at the core of any signal processing framework, and a general and formal notion of convolution is captured in algebraic signal processing (ASP) exploiting the concepts of representation theory of algebras~\cite{algSP0, algSP1, algSP2, algSP3}. Any ASP is determined by the triple 

%
%
\begin{equation}\label{eqn_ASP_signal_model}
   (\ccalA,\ccalV,\rho),
\end{equation}   
%
%

where $\ccalA$ is an associative unital algebra, $\ccalV$ is a vector space and $\rho:\ccalA\rightarrow\text{End}(\ccalV)$ is a homomorphism. The pair $(\ccalV,\rho)$ is known as a \textit{representation} of $\ccalA$. The signals are elements of $\ccalV$ while the filters are elements of $a\in\ccalA$ and its realization is given by $\rho(a)\in\End{V}$. The \textit{convolution} between a signal $\bbx\in\ccalV$ and a filter $a\in\ccalA$ is defined as the action of $a$ on $\ccalV$, this is

%
%
\begin{equation}\label{eqn_ASP_filter_outputs}
   \bby = \rho(a) \bbx.
\end{equation}   
%
%

While the algebra $\ccalA$ defines the types of operations or laws that govern the signal model, $\rho(a)$ provides their realization and therefore it indicates \textit{how} such operations are performed. Particular instantiations of eqn.~(\ref{eqn_ASP_signal_model}) lead to well known signal processing models such as 
discrete time signal processing (DTSP)~\cite{algSP0}, graph signal processing (GSP)~\cite{dsp_graphsmoura}, graphon signal processing (WSP)~\cite{ruiz2020graphon}, group signal processing (Group-NN)~\cite{algSP0}, signal processing on sets~\cite{puschel_dsponsets}, quiver signal processing~\cite{parada_quiversp}, among others.
 
Any element in $\ccalA$ can be represented in terms of the \textit{generators} of $\ccalA$, which we formally introduce in the following definition.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   D   E   F   I   N   I   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%

\begin{definition}[Generators] \label{def_generators} For an associative algebra with unity $\ccalA$ we say the set $\ccalG\subseteq\ccalA$ generates $\ccalA$ if all $a\in\ccalA$ can be represented as polynomial functions of the elements of $\ccalG$. We say elements $g\in\ccalG$ are generators of $\ccalA$ and we denote as $a=p_{\ccalA}(\ccalG)$ the polynomial that generates $a$.
\end{definition}

Since the homomorphism $\rho$ preserves the products in $\ccalA$, the elements in the image of $\ccalA$ under $\rho$ can be written as functions of the images of the generators, which are called \textit{shift operators} and whose formal definition is stated as follows.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   D   E   F   I   N   I   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{definition}[Shift Operators]\label{def_shift_operators} 
Let $(\ccalV,\rho)$ be a representation of the algebra $\ccalA$. Then, if $\ccalG\subset\ccalA$ is a generator set of $\ccalA$, the operators $\bbS = \rho(g)$ with $g\in\ccalG$ are called shift operators. The set of all shift operators is denoted by $\ccalS$
\end{definition}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

If $p\in\ccalA$ is generated by the elements in the set $\ccalG\subset\ccalA$ we denote this by $p(g)$ where $g\in\ccalG$, and we represent the image of $p(g)$ in $\End{V}$ as $p(\bbS)$ where $\bbS=\rho(g)$.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%  EXAMPLE  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{example}[GSP]\normalfont
Let $(\ccalA,\ccalV,\rho)$ be the algebraic signal model where $\ccalA=\mathbb{C}[t]$ is the univariate polynomial algebra generated by $t$, and $\ccalV=\mathbb{R}^{N}$ is the set of functions supported on the nodes of a graph $G$ with $N$ vertices and adjacency (weight) matrix $\bbW$. Then, if the homomorphism $\rho$ is selected such that $\rho(t)=\bbS=\bbW$, we have the traditionally used \textit{graph signal processing (GSP)} model. Then, the filtering (convolution) of a signal $\bbx\in\ccalV$ by the filter $p(t)=(t^{2}+t)\in\mathbb{C}[t]$ is given by $\rho(p(t))\bbx=\bbW^{2}\bbx+\bbW\bbx$.
\end{example}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%  EXAMPLE  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{example}[DSP]\normalfont
Let $(\ccalA,\ccalV,\rho)$ be the algebraic signal model where $\ccalA=\mathbb{C}[t]/(t^{N}-1)$, this is the algebra of polynomials modulo $t^{N}-1$,  $\ccalV=\mbC^N$ and $\rho$ given according to $\rho(t)=\bbC$ where $\bbC$ is the cyclic shift used for discrete signals in the $N-$dimensional space, with $\bbC^{N}=\bbI$. Then, the filtering of a signal $\bbx\in\ccalV$ by means of a filter $p(t)= \sum_{k=0}^{K-1} h_k t^k$ is given by
%
$
\rho(p(t))\bbx= \sum_{k=0}^{K-1} h_k \bbC^k\bbx.
$
%
\end{example}









==> v13/sec_SpectOP.tex <==
%!TEX root = journal_AlgNN_v08.tex

\section{Spectral Operators}\label{sec:spectopt}
Before we proof the theorems presented in previous section, it is important to discuss the concept of \textit{Fourier decomposition} in the context of representation theory of algebras. We want to highlight specially the role of the filters when a representation is compared to its perturbed version. In particular, we will show that there are essentially two factors that can cause  differences between operators and their perturbed versions, the eigenvalues\footnote{As we will show later, this is indeed a particular case of a general notion of homomorphism between the algebra and an irreducible subrepresentation of $\mathcal{A}$.} and eigenvectors. Additionally, we show how the algebra can only affect one of those sources. This is consistent with the fact that differences in the eigenvectors of the operators only affect the constants that are associated to the stability bounds.

We highlight that the concept of spectral decomposition exploited extensively in traditional signal processing can be considered as a particular case of the concept of direct sums\footnote{When considering representations of non-compact groups this concept is insufficient and it is replaced for the more general notion of \textit{direct integral of Hilbert spaces}~\cite{folland2016course,deitmar2014principles}} of \textit{irreducible} representations. In this section we provide some basic definitions from the representation theory of algebras and its connection with the notion of spectral decomposition of signals in algebraic neural networks.  This will be useful and necessary in Section~\ref{sec:proofofTheorems} as the norm of the operators considered can be calculated in the terms of an spectral representation. We start with the following definition.
%%
%%------------------------Subsection---------------------------------
%\subsection{Finite and Countable infinite Dimensional Representations}
\begin{definition}
Let $(\mathcal{M},\rho)$ be a representation of $\mathcal{A}$. Then, a representation $(\mathcal{U},\rho)$ of $\mathcal{A}$ is a \textbf{subrepresentation} of  $(\mathcal{M},\rho)$ if $\mathcal{U}\subseteq\mathcal{M}$ and $\mathcal{U}$ is invariant under all operators $\rho(a)~\forall~a\in\mathcal{A}$, i.e. $\rho(a)u\in\mathcal{U}$ for all $u\in\mathcal{U}$ and $a\in\mathcal{A}$. A representation $(\mathcal{M}\neq 0,\rho)$ is \textbf{irreducible} or simple if the only subrepresentations of $(\mathcal{M}\neq 0,\rho)$ are $(0,\rho)$ and $(\mathcal{M},\rho)$.
\end{definition}
%
The class of irreducible representations of an algebra $\mathcal{A}$ is denoted by $\text{Irr}\{\mathcal{A}\}$. Notice that the zero vector space and $\mathcal{M}$ induce themselves subrepresentations of $(\mathcal{M},\rho)$. In order to state a comparison between representations the concept of \textit{homomorphism between representations} is introduced in the following definition.
%%
%%------------------------ Definition -----------------------------------------
\begin{definition}\label{def:homrep}
Let $(\mathcal{M}_{1},\rho_{1})$ and $(\mathcal{M}_{2},\rho_{2})$ be two representations of an algebra $\mathcal{A}$. A homomorphism or \textbf{interwining operator} $\phi:\mathcal{M}_{1}\rightarrow\mathcal{M}_{2}$ is a linear operator which commutes with the action of $\mathcal{A}$, i.e.
\begin{equation}
\phi(\rho_{1}(a)v)=\rho_{2}(a)\phi(v).
\label{eq:interwinop}
\end{equation}
A homomorphism $\phi$ is said to be an isomorphism of representations if it is an isomorphism of vectors spaces. 
\end{definition}
%%
%%
Notice from definition~\ref{def:homrep}  a substantial difference between the concepts of isomorphism of vector spaces and  isomorphism of representations. In the first case we can consider that two arbitray vector spaces of the same dimension (finite) are isomorphic, while for representations that condition is required but still the condition in eqn.~(\ref{eq:interwinop}) must be satisfied. For instance, as pointed out in~\cite{repthysmbook} all the irreducible 1-dimensional representations of the polynomial algebra $\mathbb{C}[t]$ are non isomorphic.

As we have discussed before, the vector space $\mathcal{M}$ associated to $(\mathcal{M},\rho)$  provides the space where the signals are modeled. Therefore, it is of central interest to determine whether it is possible or not to \textit{decompose} $\mathcal{M}$ in terms of simpler or smaller spaces consistent with the action of $\rho$.  We remark that for any two representations $(\mathcal{M}_{1},\rho_{1})$ and $(\mathcal{M}_{2},\rho_{2})$ of an algebra $\mathcal{A}$, their direct sum is given by the representation $(\mathcal{M}_{1}\oplus\mathcal{M}_{2},\rho)$ where $\rho(a)(\mathbf{x}_{1}\oplus\mathbf{x}_{2})=(\rho_{1}(a)\mathbf{x}_{1}\oplus\rho_{2}(a)\mathbf{x}_{2})$. We introduce the concept of indecomposability in the following definition.
%%
%%------------------------ Definition ------------------------------------------
\begin{definition}\label{def:indecomprep}
A nonzero representation $(\mathcal{M},\rho)$ of an algebra $\mathcal{A}$ is said to be \textbf{indecomposable} if it is not isomorphic to a direct sum of two nonzero representations.
\end{definition}
%%
%%
Indecomposable representations provide the \textit{minimum units of information} that can be extracted from signals in a given space when the filters have a specific structure (defined by the algebra)~\cite{barot2014introduction}. The following theorem provides the basic building block for the decomposition of finite dimensional representations.
%%
%%-----------------------------Theorem-------------------------------------------
\begin{theorem}[Krull-Schmit, \cite{repthybigbook}]\label{theorem:krullschmitdecomp}
Any finite dimensional representation of an algebra can be decomposed into a finite direct sum of indecomposable subrepresentations and this decomposition is unique up to the order of the summands and up to isomorphism. 
\end{theorem}
%%
%%
The uniqueness in this result means that if $(\oplus_{r=1}^{r}V_{i},\rho)\cong(\oplus_{j=1}^{s}W_{j},\gamma)$ for indecomposable representations $(V_{j},\rho_{j}),(W_{j},\gamma_{j})$, then $r=s$ and there is a permutation $\pi$ of the indices such that $(V_{i},\rho_{i})\cong (W_{\pi(j)},\gamma_{\pi(j)})$~\cite{repthybigbook}. Although theorem~\ref{theorem:krullschmitdecomp} provides the guarantees for the decomposition of representation in terms of indecomposable representations, it is not applicable when infinite dimensional representations are considered. However, it is possible to overcome this obstacle taking into account that irreducible representations are indecomposable~\cite{repthysmbook,repthybigbook}, and they can be used then to build representations that are indecomposable. In particular, \textit{irreducibility} plays a central role to decompose the invariance properties of the images of $\rho$ on $\text{End}(\mathcal{M})$~\cite{repthybigbook}. Representations that allow a decomposition in terms of subrepresentations that are irreducible are called \textit{completely reducible} and its formal description is presented in the following definition.
%%
%%-----------------------------Definition-----------------------------------------
\begin{definition}[~\cite{repthybigbook}]\label{def:complredu}
 A representation $(\mathcal{M},\rho)$ of the algebra $\mathcal{A}$ is said to be \textbf{completely reducible} if $(\mathcal{M},\rho)=\bigoplus_{i\in I}(\mathcal{U}_{i},\rho_{i})$ with irreducible subrepresentations $(\mathcal{U}_{i},\rho_{i})$. The \textbf{length} of $(\mathcal{M},\rho)$ is given by $\vert I\vert$.
\end{definition}
%%
%%
%Irreducible representations are indecomposable, therefore by using irreducible representations it is possible to decompose an arbitrary representation where the minimum component in the decomposition has an \textit{invariance property}.  

For a given $(\mathcal{U},\rho_{\mathcal{U}})\in\text{Irr}\{\mathcal{A}\}$ the sum of all irreducible subrepresentations of $(V,\rho_{V})$ that are equivalent (isomorphic) to $(\mathcal{U},\rho_{\mathcal{U}})$ is represented by $V(\mathcal{U})$ and it is called the $\mathcal{U}$-homogeneous component of $(V,\rho_{V})$. This sum is a direct sum, therefore it has a length that is well defined and whose value is called the \textit{multiplicity} of $(\mathcal{U},\rho_{\mathcal{U}})$ and is represented by $m(\mathcal{U},V)$~\cite{repthybigbook}. Additionally, the sum of all irreducible subrepresentations of $(V,\rho_{V})$ will be denoted as $\text{soc}\{V\}$. It is possible to see that a given representation $(V,\rho_{V})$ is completely reducible if and only if $(V,\rho_{V})=\text{soc}\{S\}$~\cite{repthybigbook}. The connection between $\text{soc}\{V\}$ and $V(\mathcal{U})$ is given by the following proposition. 
%%
%%---------------------------Proposition-------------------------------------
\begin{proposition}[Proposition 1.31~\cite{repthybigbook}]\label{prop:repdirectsum1}
Let $(V,\rho_{V})\in\mathsf{Rep}\{A\}$. Then $\text{soc}\{V\}=\bigoplus_{S\in\text{Irr}\{\mathcal{A}\}}V(S)$.
\end{proposition}
%%
%%
Now, taking into account that any homogeneous component $V(\mathcal{U})$ is itself a direct sum we have that 
\begin{equation}
\text{soc}\{V\}\cong\bigoplus_{S\in\text{Irr}\{\mathcal{A}\}}S^{\oplus m(\mathcal{U},V)}.
\label{eq:repdirectsumtot}
\end{equation}
Equation~(\ref{eq:repdirectsumtot}) provides the building block for the definition of Fourier decompositions in algebraic signal processing~\cite{algSP1}. With all these concepts at hand we are ready to introduce the following definition.
%%
%%-----------------------------Definition------------------------------------------
\begin{definition}[Fourier Decomposition]\label{def:foudecomp}
For an algebraic signal model $(\mathcal{A},\mathcal{M},\rho)$ we say that there is a spectral or Fourier decomposition of $(\mathcal{M},\rho)$ if
\begin{equation}
(\mathcal{M},\rho)\cong\bigoplus_{(\mathcal{U}_{i},\phi_{i})\in\text{Irr}\{\mathcal{A}\}}(\mathcal{U}_{i},\phi_{i})^{\oplus m(\mathcal{U}_{i},\mathcal{M})}
 \label{eq:foudecomp1}
\end{equation}
where the $(\mathcal{U}_{i},\phi_{i})$ are irreducible subrepresentations of $(\mathcal{M},\rho)$. Any signal $\mathbf{x}\in\mathcal{M}$ can be therefore represented by the map $\Delta$ given by 
\begin{equation}
\begin{matrix} 
\Delta: & \mathcal{M} \to \bigoplus_{(\mathcal{U}_{i},\phi_{i})\in\text{Irr}\{\mathcal{A}\}}(\mathcal{U}_{i},\phi_{i})^{\oplus m(\mathcal{U}_{i},\mathcal{M})} \\ & \mathbf{x}\mapsto \hat{\mathbf{x}}
 \end{matrix}
 \label{eq:foudecomp2}
\end{equation}
known as the Fourier decomposition of $\mathbf{x}$ and the projection of $\hat{\mathbf{x}}$ in each $\mathcal{U}_{i}$ are the Fourier components represented by $\hat{\mathbf{x}}(i)$.
\end{definition}
%%
%%
%\begin{figure}
% \centering\includegraphics[scale=1,angle=0]{../figures/fig9.pdf}
%  \caption{Diagram indicating the maps and the spaces when a completely reducible representation $(\mathcal{M},\rho)$ is decomposed as a direct sum of irreducible subrepresentations.}
%  \label{fig_3}
%\end{figure}
%%
%%
Notice that in eqn.~(\ref{eq:foudecomp1}) there are two sums, one dedicated to the non isomorphic subrepresentations (external) and another one (internal) dedicated to subrepresentations that are isomorphic. In this context, the sum for non isomorphic representations indicates the sum on the \textit{frequencies} of the representation while the sum for isomorphic representations a sum of components associated to a given frequency. It is also worth pointing out that $\Delta$ is an interwining operator, therefore, we have that $\Delta(\rho(a)\mathbf{x})=\rho(a)\Delta(\mathbf{x})$. As pointed out in~\cite{algSP0} this can be used to define a convolution operator as $\rho(a)\mathbf{x}=\Delta^{-1}(\rho(a)\Delta(\mathbf{x}))$. The projection of a filtered signal $\rho(a)\mathbf{x}$ on each $\mathcal{U}_{i}$ is given by $\phi_{i}(a)\hat{\mathbf{x}}(i)$ and the collection of all this projections is known as the \textit{spectral representation} of the operator $\rho(a)$. Notice that $\phi_{i}(a)\hat{\mathbf{x}}(i)$ translates to different operations depending on the dimension of $\mathcal{U}_{i}$. For instance, if $\text{dim}(\mathcal{U}_{i})=1$, $\hat{\mathbf{x}}(i)$ and $\phi_{i}(a)$ are scalars while if $\text{dim}(\mathcal{U}_{i})>1$ and finite $\phi_{i}(a)\hat{\mathbf{x}}(i)$ is obtained as a matrix product.
%
%
%In many important applications the $\mathcal{U}_{i}$ in eqn.~(\ref{eq:foudecomp1}) are one dimensional spaces~\cite{algSP0,algSP1,algSP3}, that when seen as homogeneous components of a representation $(V,\rho_{V})$  became of particular interest as they are connected with the traditional concepts of eigenspaces and eigenvalues~\cite{repthybigbook}. Indeed, eigenspaces can be considered particular cases of the so called \textit{weight spaces}, introduced in the following definition.
%%%
%%%---------------------------Definition-----------------------------------------
%\begin{definition}[Weight spaces~\cite{repthybigbook}]\label{def:weightspaces}
%Let $(\mathcal{U},\phi)$ be a 1-dimensional representation of an algebra $\mathcal{A}$. Then the $\mathcal{U}-$homogeneous component $V(\mathcal{U})$ is given by
%\begin{equation}
%V(\mathcal{U})=\left\lbrace v\in V\vert \rho(a)v=\phi(a)v~\forall~a\in\mathcal{A}\right\rbrace 
%\label{eq:weightspaces}
%\end{equation}
%if $V(\mathcal{U})\neq 0$, then $\phi$ is called a \textbf{weight} of the representation $(V,\rho_{V})$ and $V(\mathcal{U})$ is called the corresponding \textbf{weight space}.
%\end{definition}
%%%
%%%
%In the context of definition~\ref{def:weightspaces} it is important to point out that when $\mathcal{A}=\mathbb{K}[t]$ and  $\phi(t)=\lambda\in\mathbb{K}$, $V(\mathcal{U})$ is the usual eigenspace for the eigenvalue $\lambda$ of the endomorphism $\rho(t)$. However when the algebra is not polynomial eqn.(~\ref{eq:weightspaces}) offers a generalization that allows to define more general spectral representations. 

%When considering definition~(\ref{def:foudecomp}) and eqn.(\ref{eq:foudecomp2}) with one dimensional subrepresentations the spectral representation of the operator $\rho(a)$ is given by
%\begin{equation}
%\rho(a)\mathbf{x}=\sum_{i}\hat{\mathbf{x}}(i)\phi_{i}(a)\mathbf{u}_{i}
%\label{eq:spectopt}
%\end{equation}
%where $\mathbf{u}_{i}$ is the basis vector associated to $\mathcal{U}_{i}$.
%%
%%-------------------------Remark--------------------------------------------------------------
\begin{remark}\label{remark:interpSpecFilt}\normalfont
The spectral representation of an operator indicated as $\phi_{i}(a)\hat{\mathbf{x}}(i)$ and eqns.~(\ref{eq:foudecomp1}) and~(\ref{eq:foudecomp2}) highlight one important fact that is essential for the discussion of the results in Section~\ref{sec:proofofTheorems}. For a completely reducible representation $(\mathcal{M},\rho)\in\mathsf{Rep}\{\mathcal{A}\}$ the connection between the algebra $\mathcal{A}$ and the spectral representation is \textit{exclusively} given by $\phi_{i}(a)$ which is acting on $\hat{\mathbf{x}}(i)$, therefore, it is not possible by the selection of elements or subsets of the algebra to do any modification on the spaces $\mathcal{U}_{i}$ associated to the irreducible components in eqn.(\ref{eq:foudecomp1}). As a consequence, when measuring the similarities between two operators $\rho(a)$ and $\tilde{\rho}(a)$ associated to $(\mathcal{M},\rho)$ and $(\mathcal{M},\tilde{\rho})$, respectively, there will be two sources of error. One source of error that can be modified by the selection of $a\in\mathcal{A}$ and another one that will be associated with the differences between spaces $\mathcal{U}_{i}$ and $\tilde{\mathcal{U}}_{i}$, which are associated to the direct sum decomposition of $(\mathcal{M},\rho)$ and $(\mathcal{M},\tilde{\rho})$, respectively. This point was first elucidated in~\cite{fern2019stability} for the particular case of GNNs, but it is part of a much more general statement that becomes more clear in the language of algebraic signal processing. 
\end{remark}
%%
%%
%%------------------------------Subsection----------------------------
%%
%\subsection{Examples}
%%
%\subsubsection{CNNs}
\begin{example}[Discrete signal processing]\normalfont
In CNNs the filtering is defined by the polynomial algebra $\mathcal{A}=\mathbb{C}[t]/(t^{N}-1)$, therefore, in a given layer the spectral representation of the filters is given by
%
\begin{multline*}
\rho(a)\mathbf{x}=\sum_{i=1}^{N}\phi_{i}\left(\sum_{k=0}^{K-1}h_{k}t^{k}\right)\hat{\mathbf{x}}(i)\mathbf{u}_{i}\\
=\sum_{i=1}^{N}\sum_{k=0}^{K-1}h_{k}\phi_{i}(t)^{k}\hat{\mathbf{x}}(i)\mathbf{u}_{i}
=\sum_{i=1}^{N}\sum_{k=0}^{K-1}h_{k}\left(e^{-\frac{2\pi ij}{N}}\right)^{k}\hat{\mathbf{x}}(i)\mathbf{u}_{i},
\end{multline*}
%
with $a=\sum_{k=0}^{K-1}h_{k}t^{k}$ and where the $\mathbf{u}_{i}(v)=\frac{1}{\sqrt{N}}e^{\frac{2\pi jvi}{N}}$ are the column vectors of the traditional DFT matrix, while $\phi_{i}(t)=e^{-\frac{2\pi ji}{N}}$ is the eigenvalue associated to $\mathbf{u}_{i}$. Here $\hat{\mathbf{x}}$ represents the DFT of $\mathbf{x}$.
\end{example}
%%
%%---------------------------------Subsection-----------------------------------
\begin{example}[Graph signal processing]\normalfont
Taking into account that the filtering in each layer of a GNN is defined by a polynomial algebra, the spectral representation of the filter is given by
%
\begin{multline}
\rho(a)\mathbf{x}=\sum_{i=1}^{N}\phi_{i}\left(\sum_{k=0}^{K-1}h_{k}t^{k}\right)\hat{\mathbf{x}}(i)\mathbf{u}_{i}\\
=\sum_{i=1}^{N}\sum_{k=0}^{K-1}h_{k}\phi_{i}(t)^{k}\hat{\mathbf{x}}(i)\mathbf{u}_{i}=
\sum_{i=1}^{N}\sum_{k=0}^{K-1}h_{k}\lambda_{i}^{k}\hat{\mathbf{x}}(i)\mathbf{u}_{i}
\label{eq:specopgnn}
\end{multline}
%
with $a=\sum_{k=0}^{K-1}h_{k}t^{k}$, and where the $\mathbf{u}_{i}$ are given by the eigenvector decomposition of $\rho(t)=\mathbf{S}$, where $\mathbf{S}$ could be the adjacency matrix or the Laplacian of the graph, while $\phi_{i}(t)=\lambda_{i}$ being $\lambda_{i}$ the eigenvalue associated to $\mathbf{u}_{i}$. The projection of $\mathbf{x}$ in each subspace $\mathcal{U}_{i}$ is given by $\hat{\mathbf{x}}(i)=\langle\mathbf{u}_{i}, \mathbf{x}\rangle$, and if $\mathbf{U}$ is the matrix of eigenvectors of $\mathbf{S}$ we have the widely known representation $\hat{\mathbf{x}}=\mathbf{U}^{T}\mathbf{x}$~\cite{gamagnns}.
\end{example}
%%
%%-------------------Example--------------------------------
\begin{example}[Group signal processing]\label{example:specopGroupCNNs}
\normalfont
Considering the Fourier decomposition on  general groups~\cite{steinbergrepg,terrasFG,fulton1991representation}, we obtain the spectral representation of the algebraic filters as
\begin{equation*}
\boldsymbol{a}\ast\mathbf{x}=\sum_{u,h\in G}\boldsymbol{a}(uh^{-1})\sum_{i,j,k}\frac{d_{k}}{\vert G\vert}\hat{\mathbf{x}}\left(\boldsymbol{\varphi}^{(k)}\right)_{i,j}\boldsymbol{\varphi}_{i,j}^{(k)}(h)hu,
\end{equation*}
where $\hat{\mathbf{x}}(\boldsymbol{\varphi}^{(k)})$ represents the Fourier components associated to the $k$th irreducible representation with dimension $d_{k}$ and $\boldsymbol{\varphi}^{(k)}$ is the associated unitary element. We can see that the $k$th element in this decomposition is $\sum_{i,j}\mathbf{x}(\varphi^{(k)})_{i,j}\sum_{u,h}\frac{d_{k}}{\vert G\vert}\boldsymbol{a}(uh^{-1})\boldsymbol{\varphi}_{i,j}^{(k)}(h)hu$.
\end{example}
%%
%%-------------------Subsection--------------------------------
%\subsubsection{CNNs, with infinite dimensional representations}
\begin{example}[Graphon signal processing]\normalfont
According to the spectral theorem~\cite{conway1994course,aliprantis2002invitation}, it is possible to represent the action of a compact normal operator $S$ as $S\mathbf{x}=\sum_{i}\lambda_{i}\langle\boldsymbol{\varphi}_{i},\mathbf{x}\rangle\boldsymbol{\varphi}_{i}$ where $\lambda_{i}$ and $\boldsymbol{\varphi}_{i}$ are the eigenvalues and eigenvectors of $S$, respectively, and $\langle\cdot\rangle$ indicates an inner product. Then, the spectral representation of the filtering of a signal in the layer $\ell$ is given by
\begin{equation*}
\rho_{\ell}\left(p(t)\right)\mathbf{x}
=
\sum_{i}p(\lambda_{i})\langle\mathbf{x},\boldsymbol{\varphi}_{i}\rangle\boldsymbol{\varphi}_{i}=\sum_{i}\phi_{i}(p(t))\hat{\mathbf{x}}_{i}\boldsymbol{\varphi}_{i},
\end{equation*}
where $\phi_{i}(p(t))=p(\lambda_{i})$.
\end{example}










==> v13/sec_aggalgnn.tex <==
%!TEX root =../compiler_paper.tex




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure*}
 \centering\includegraphics[scale=1,angle=0]{../figures/fig15c.pdf}
 \caption{Schematic representation of how the information is processed in an Agg-AlgNN that posses two layers in the regular CNN processing stage. First a signal $x\in\ccalV$ is mapped into $\ccalV_{1}=\oplus_{i=1}^{\text{dim}(\ccalV)}\ccalV$ as $\bbR(x)=\tilde{x}=\oplus_{i=0}^{m}x$. Then $\tilde{x}$ is filtered by the shift operator $\rho_{1}(g)=\bbS_{1}=\oplus_{i=0}^{m}\bbS^{i}_{0}$ leading to $\oplus_{i=0}^{m}\bbS_{0}^{i}x$, which is processed with the signal model $(\ccalA,\ccalM_{1},\rho_{2})$.}
 \label{fig_1}
\end{figure*}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%

\section{Aggregation Algebraic Neural Networks} \label{sec_aggalgnn}

In this section we extend and generalize the results presented for Agg-GNNs. We start reviewing the basics about algebraic signal processing.

%%---------------------------------------------------------------------
%%---------------- Subsection Algebraic Signal processing
%%---------------------------------------------------------------------

\input{\pathsections/sec_RTASM.tex}




An aggregation algebraic neural network  is composed of two stages of processing, an aggregation stage and a CNN stage. In the aggregation stage an arbitrary signal model is used to leverage properties of the signal and its domain, and second there is a stage where information is processed be means of a traditional CNN which is defined by algebraic signal models associated to discrete signal processing. In what follows we discuss with full detail each processing stage.




\subsection{Aggregation stage and Aggregation Operator}


The aggregation stage is defined in terms of the aggregation operator, that we introduce in the following definition.

 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   D   E   F   I   N   I   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%

\begin{definition}[Aggregation Operator] \label{def_aggoperator} 
Let $(\ccalA,\ccalV,\rho)$ be an algebraic signal model with shift operators $\{\bbS_{i}\}_{i=1}^{m}$. Then, if $\ccalM_{k}$ denotes the set of monomials on  $\{\bbS_{i}\}_{i=1}^{m}$ whose degree equals $k$, we say that the \textbf{aggregation operator}, $\bbA$, of order $a$ is given  by
%
%
\begin{equation}
\bbA(\bbx)=\bbx
                    \bigoplus_{p_{1}\in\ccalM_{1}}p_{1}\bbx
                    \bigoplus_{p_{2}\in\ccalM_{2}}p_{2}\bbx
                    \bigoplus
                    \cdots
                    \bigoplus_{p_{a}\in\ccalM_{a}}p_{a}\bbx
\end{equation}
%
%
\end{definition}


Before we continue our discussion we present some examples of aggregation operators in light of Definition~\ref{def_aggoperator}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%  EXAMPLE  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{example}\normalfont
Let $(\ccalA,\ccalV,\rho)$ be an algebraic signal model with shift operators $\bbS_{1}$ and $\bbS_{2}$ and where $\ccalA$ is non commutative. Then, the application of the aggregation operator of order 2 on $\bbx\in\ccalV$ is given according to
%
%
\begin{equation}
\bbA(\bbx)=
                         \bbx
                         \oplus\bbS_{1}\bbx
                         \oplus\bbS_{2}\bbx
                         \oplus\bbS_{1}^{2}\bbx
                         \oplus\bbS_{2}^{2}\bbx
                         \oplus\bbS_{1}\bbS_{2}\bbx  
                         \oplus\bbS_{2}\bbS_{1}\bbx 
\end{equation}
%
%
\end{example}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%  EXAMPLE  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{example}\normalfont
Let $(\mathbb{C}[t],\mathbb{R}^{N},\rho)$ be the GSP signal model for the processing of signals on a graph $G$.  $\mathbb{C}[t]$ is the univariate polynomial algebra on $t$ and complex coefficients and $\rho(t)=\bbS$ where $\bbS$ is the adjacency matrix of $G$. Then, the aggregation operator of order $3$ is given by
%
%
\begin{equation}
\bbA(\bbx)=
                         \bbx
                         \oplus\bbS\bbx
                         \oplus\bbS^{2}\bbx
                         \oplus\bbS^{3}\bbx
\end{equation}
%
%

It is worth pointing out, that the action of the aggregation operator on $\bbx$ represented above is equivalent to the traditional representation on aggregation GNNs  given by

%
%
\begin{equation}\label{eq:agggnns}
\bbA(\bbx)= 
                   \left[ 
                          \bbx,\bbS\bbx, \bbS^{2}\bbx,\bbS^{3}\bbx
                   \right],
\end{equation}
%
%
this is, the operator $\bbA$ embeds filtrated versions of $\bbx$ into the columns of a matrix.
\end{example}








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%  MAIN MATTER  %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






\medskip
The aggregation stage is simply the application of the aggregation operator. It is worth pointing out that the aggregation operator maps any signal, $\bbx$, into a new signal that exhibits directly properties of $\bbx$ highlighted by the successive application of the shift operators, which additionally can be associated with another shift operator in a higher dimensional space. To illustrate this, let us consider Figure~\ref{fig_1} that illustrates an Agg-AlgNN whose aggregation stage is based on an algebraic signal model $(\ccalA,\ccalV,\rho)$ and where the algebra posses a single generator $g$. As indicated in Fig.~(\ref{fig_1}) the aggregation operator $\bbA$ of order $a$ can be expressed as the composition of two operators, $\bbG$ and $\bbS_{Agg}$, where $\bbG:\ccalV\to\bigoplus_{i=0}^{a}\ccalV$ replicates the signal $\bbx$ a number of $a+1$ times, i.e. $\bbG(\bbx)=\oplus_{i=0}^{a}\bbx$, and $\bbS_{Agg}$ is a shift operator for the signal model $\left(\ccalA,\bigoplus_{i=0}^{a}\ccalV,\rho_{Agg}\right)$ where $\rho_{Agg}(t)=\bbS_{Agg}=\bbI\oplus\bbS\oplus\bbS^{2}\oplus\cdots\oplus\bbS^{a}$. The action of $\bbS_{Agg}$ on $\bbG(\bbx)$ is then given by $\rho_{Agg}(t)\bbG(\bbx)=\bbx\oplus\bbS\bbx\oplus\bbS^{2}\bbx\oplus\cdots\oplus\bbS^{a}\bbx$.



\subsection{Regular CNN processing}

Once the information is processed with the aggregation operator, the resultant quantity is mapped to a regular CNN stage via the operator $\bbQ$ (see Fig.~\ref{fig_1}) that permutes the information. In the CNN stage information is processed with signal models obtained from representations of the algebra $\ccalC=\bigoplus_{i=1}^{\text{dim}\left(\ccalV\right)}\mathbb{C}[t]$. Notice that the product between two elements $\oplus_{i=1}^{\text{dim}(\ccalV)}a_{i}\in\ccalC$ and $\oplus_{i=1}^{\text{dim}(\ccalV)}b_{i}\in\ccalC$ is given by $\oplus_{i=1}^{\text{dim}(\ccalV)}a_{i}b_{i}$, and the generator element of $\ccalC$ is $\oplus_{i=1}^{\text{dim}(\ccalV)}t$ where $t$ is the generator of $\mathbb{C}[t]$.





%%--------------------------------------------------
%%---------REMARK----------------------------
%%--------------------------------------------------

\begin{remark}\normalfont
It is worth pointing out that in the traditional notation of aggregation GNNs the regular CNN stage process with regular CNNs \textit{each row} of the matrix in eqn.~(\ref{eq:agggnns}). The operator $\bbQ$ is a mere indication that the information is processed by rows.  
\end{remark}






Of particular importance is the first layer of the CNN after the aggregation stage, whose signal model is given by
 
 %
 %
 \begin{equation}
 \left( 
        \bigoplus_{i=1}^{ \text{dim} \left(\ccalV \right) }\mathbb{C}[t], 
         \bigoplus_{i=1}^{\text{dim}(\ccalV)}\ccalR_{i}^{(1)},
         \phi_{1}
\right)
 \end{equation}
%
%
 with
%
%
$
\phi_{1}\left(\oplus_{i=1}^{\text{dim}(\ccalV)}t\right)=\oplus_{i=1}^{\text{dim}(\ccalV)}\bbC_{0\vert (a+1)}, \ccalR_{i}^{(1)}\cong\mathbb{R}^{a+1}
$
%
%
and where $\bbC_{0\vert (a+1)}$ is the shift operator used in traditional DSP acting on discrete signals of dimension $a+1$, this is the shift operator in the algebraic signal model $(\mathbb{C}[t], \mathbb{C}^{a+1}, \theta)$, where $\theta(t)=\bbC_{0\vert (a+1)}$.

The mapping between the aggregation layer is dictated by the operator $\bbQ: \bigoplus_{i=0}^{a}\ccalV \to \bigoplus_{i=1}^{\text{dim}(\ccalV)}\mathcal{R}_{i}^{(1)}$, whose restriction on $\mathcal{R}_{i}^{(1)}$ is given by

%
%
\begin{equation}
\left.\bbQ
       \left(  \oplus_{j=0}^{a}\bbS^{j}\bbx  \right)\right\vert_{\mathcal{R}_{i}^{(1)}} 
                          =\bbr_{i},\quad
                          \text{with}\quad 
                          \left[\bbr_{i}\right]_{\ell}=\left[\bbS^{\ell}\bbx\right]_{i},\quad 0\leq\ell\leq a,
\end{equation}
%
%
where $[\bbb]_{\ell}$ represents the $\ell$th component of a given vector $\bbb$.

In the CNN, the information is mapped from the layer $\ell$ to the layer $\ell+1$ by means of Lipschitz maps $\sigma_{\ell}: \ccalR_{i}^{(\ell)} \to \ccalR_{i}^{(\ell+1)}$, which are the composition of a pooling operator and a point wise nonlinearity function. 


From the second layer up to the last layer of the CNN, the signal processing model is given by

%
%
 \begin{equation}
 \left( 
        \bigoplus_{i=1}^{\text{dim}\left(\ccalV\right)}\mathbb{C}[t], 
         \bigoplus_{i=1}^{\text{dim}(\ccalV)}\ccalR_{i}^{(\ell)},
         \phi_{\ell}
 \right)
 \end{equation}
%
%
 with
%
%
$
\phi_{\ell}\left(\oplus_{i=1}^{\text{dim}(\ccalV)}t\right)=\oplus_{i=1}^{\text{dim}(\ccalV)}\bbC_{0\vert \text{dim}(\ccalR_{i}^{(\ell)})}.
$
%
%
In the layer $\ell$ the value $\text{dim}\left(\ccalR_{i}^{(\ell)}\right)$ is determined by the map $\sigma_{\ell-1}$, and unlike the case of the first layer of the CNN, it is not attached to the number of aggregations $a$.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
 \centering\includegraphics[scale=1,angle=0]{../figures/fig16.pdf}
 \caption{Pictorial illustration of how the information is mapped from the aggregation stage to the CNN stage. Notice that in the context of the traditional notation of Agg-GNNs, this is a mere indication that the information of the matrix in eqn.~(\ref{eq:agggnns}) is processed by rows with a CNN.}
 \label{fig_2}
\end{figure}









\subsection{Conventions and notations for Agg-AlgNN}

In what follows we denote a generic Agg-AlgNN using the notation 
%
$\Xi=\left\lbrace
                        \left.
                               (\ccalA,\ccalV,\rho)
                        \right\vert
                                        \text{\texttt{CNN}}(L,F_{\ell})       
\right\rbrace$,
%
to indicate an Agg-AlgNN where the algebra with an algebraic signal model $ (\ccalA,\ccalV,\rho)$ in the aggregation stage, followed by a regular CNN stage with $L$ layers that used $F_{\ell}$ features per layer.








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%  EXAMPLE  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\begin{example}[Aggregation GNNs]\normalfont
%Aggregation GNNs are a particular instantiation of a generic Agg-AlgNN considering the algebraic model for GSP in the aggregation stage. In particular, the aggregation operation maps an arbitrary graph signal $\bbx$ into the matrix $\bbX$ given by
%
%%
%%
%\begin{equation*}
%\bbX=
%          \left[
%                   \bbx, \bbS\bbx, \bbS^{2}\bbx, \ldots, \bbS^{a}\bbx
%          \right].
%\end{equation*}
%%
%%
% 
%Now, if we denote by $\bbz_{r}$ the $r$th row of $\bbX$, we obtain the $g$th featues by means of traditional convolution with a filter $\bbh_{g}$ generating the signal  $\bby_{r}^{g}=\bbh_{g}\ast\bbz_{r}$.
%
%\end{example}








==> v13/sec_algNN.tex <==

%%---------------------------------------------------------------------
%%---------SECTION: ALGEBRAIC NEURAL NETWORKS -------------------------
%%---------------------------------------------------------------------



\section{Algebraic Neural Networks}
\subsection{Convolution Feaures}
\subsection{Pooling}

==> v13/sec_conclusions.tex <==
%!TEX root =../compiler_paper.tex





%
%%----------------------------------------------------------------------------
%%-------- SECTION: CONCLUSIONS --------------------------------- ------------
%%----------------------------------------------------------------------------
%%
%%------------------- Title ------------------------------
\section{Conclusions}\label{sec:conclusions}

\blue{NOTE: Here provide some conclustions}

%We considered algebraic neural networks (AlgNN) with commutative algebras as a tool to unify convolutional architectures like CNNs and GNNs, synthesizing the algebraic structure by exploiting results from the representation theory of algebras and algebraic signal processing. Within this framework, we showed that AlgNNs can, in general,  be stable to different types of perturbations, and the conditions under which the AlgNN operators are stable are determined by subsets of the algebra. We pointed out that the perturbations of the domain of the signals can be equivalently modeled as a perturbation of the representation or the signal model, and the degree of this perturbation can be measured by means of the Fr\'echet derivative of two functions, the image of the homomorhisms in $\text{End}(\mathcal{M})$ and the perturbation model $\mathbf{T}(\mathbf{S})$.  The perturbation model considered provides enough expressive power to represent a wide variety of perturbations affecting the domain of the signals or the operator themselves directly. In particular, when considering the algebraic model for GNNs, the absolute and the relative perturbation models can be considered particular cases of the perturbation model considered in this work.







==> v13/sec_perturbations.tex <==
%!TEX root = ../compiler_paper.tex




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\subsection{Perturbations}\label{sec:perturbandstability}

Taking into account that the realization of the algebraic filters in any algebraic model is given by the homomorphism, it is natural to consider the perturbation of $(\ccalA,\ccalV,\rho)$ considering changes on $\rho$. For our discussion we follow this approach pointing that, the algebra dictates the laws that define the processing strategy and therefore any change on the algebra changes the very nature of the model which is the type of modification that would go far beyond a perturbation. In the following definition we state formally the notion of perturbation considered.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   D   E   F   I   N   I   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{definition}\label{def:perturbmodel}(ASP Model Perturbation)
Let $(\ccalA,\ccalV,\rho)$ be an ASP model with algebra elements generated by $g\in\ccalG$ (Definition \ref{def_generators}) and recall the definition of the shift operators $\bbS = \rho(g)$ (Definition \ref{def_shift_operators}). We say that $(\ccalA,\ccalV,\tdrho)$ is a perturbed ASP model if for all $a=p_{\ccalA}(\ccalG)$ we have that
%
%
\begin{equation}\label{eqn_def_perturbation_model_10}
   \tdrho(a) = p_\ccalV\big(\tdrho(g)\big) 
             = p_\ccalV\big(\tilde\ccalS\big)
             =p\big(\tilde\ccalS\big),
\end{equation}
%
%
where $\tilde\ccalS$ is a set of perturbed shift operators of the form
%
%
\begin{equation}\label{eqn_def_perturbation_model_20}
   \tbS = \bbS + \bbT(\bbS),
\end{equation}
%
%
for all shift operators $\bbS\in\ccalS$. 
\end{definition}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Definition \ref{def:perturbmodel} makes specific the perturbations on the homomorphism in terms of the shift operators, allowing then a representation of any filter $\rho(a)\in\End{V}$ in terms of a map $\tilde{\rho}(a)$ which is not necessarily a homomorphism.  

As pointed out in~\cite{parada_algnn} this perturbation model allows the modeling of a rich variety of perturbations for graph signal models, discrete time signals, signals on groups, and graphon signals among others. Additionally, the perturbation on the domains of the signals can be captured by in eqn.~(\ref{eqn_def_perturbation_model_10}).





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%

\subsubsection{Perturbation Models}

In our analysis, we consider perturbations $\bbT(\bbS)$ given by

%
%
\begin{equation}\label{eqn_perturbation_model_absolute_plus_relative}
   \bbT(\bbS)=\bbT_{0} + \bbT_{1}\bbS,
\end{equation}
%
%

where $\bbT_{0}$ and $\bbT_{1}$ are compact normal operators independent from $\bbS$ with $\Vert\bbT_{r}\Vert\ll 1$.

When considering algebraic models with algebras with multiple generators $\{g_{i}\}_{i=1}^{m}$, we represent the filter $p\in\End{V}$ as a function of the shift operators $\rho(g_{i})=\bbS_{i}$, this is $p: \text{End}(\mathcal{V})^{m}\rightarrow\text{End}(\mathcal{V})$ where $\text{End}(\mathcal{V})^{m}$ is the $m$-times cartesian product of $\text{End}(\mathcal{V})$. Then, the perturbed version of the filter $p(\mathbf{S})=p(\mathbf{S}_{1},\ldots,\mathbf{S}_{m})$ is obtained as $p(\bbT(\bbS))=p\left(\mathbf{T}(\mathbf{S}_{1}),\ldots,\mathbf{T}(\mathbf{S}_{m})\right)$ where $\mathbf{T}(\mathbf{S}_{i})=\mathbf{T}_{0,i}+\mathbf{T}_{1,i}\mathbf{S}_{i}$.










 





==> v13/sec_stability.tex <==
%!TEX root = ../compiler_paper.tex





%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%

\section{Stability of Algebraic Aggregation Neural Networks}\label{sec:stabilitytheorems}



%%--------------------------------------------------------------
%%---------Subsection: Perturbartions-----------------
%%--------------------------------------------------------------
\input{\pathsections/sec_perturbations.tex}





An aggregation algebraic neural network with primary algebraic model $(\ccalA,\ccalV_{0},\rho_{0})$ can be regarded as an operator $p(\bbS)$ acting on $\ccalV_{0}$. In this section we study the stability of such operators using the notion of stability introduced in the following definition. 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   D   E   F   I   N   I   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%

\begin{definition}[Operator Stability~\cite{parada_algnn}]\label{def:stabilityoperators1} Given operators $p(\mathbf{S})$ and $p(\tilde{\mathbf{S}})$ defined on the processing models $(\ccalA,\ccalV,\rho)$ and $(\ccalA,\ccalV,\tdrho)$ (cf. Definition \ref{def:perturbmodel}) we say the operator $p(\mathbf{S})$ is Lipschitz stable if there exist constants $C_{0}, C_{1}>0$ such that 
%
%
\begin{multline}\label{eq:stabilityoperators1}
\left\Vert p(\mathbf{S})\mathbf{x}  - p(\tilde{\mathbf{S}})\mathbf{x}\right\Vert
\leq
\\
\left[
C_{0} \sup_{\bbS\in\ccalS}\Vert\mathbf{T}(\mathbf{S})\Vert + C_{1}\sup_{\bbS\in\ccalS}\big\|D_{\bbT}(\bbS)\big\|
+\mathcal{O}\left(\Vert\mathbf{T}(\mathbf{S})\Vert^{2}\right)
\right] \big\| \bbx \big\|,
\end{multline}
%
%
for all $\bbx\in\ccalM$. In \eqref{eq:stabilityoperators1} $D_{\bbT}(\bbS)$ is the Fr\'echet derivative of the perturbation operator $\bbT$. 
\end{definition}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%

Definition~\ref{def:stabilityoperators1} states that operators are stable as long as the changes in the operator are proportional to the size of the deformation or perturbation. Indeed, the right hand side of eqn.~(\ref{eq:stabilityoperators1}) represents the size of the deformation $\bbT(\bbS)$ which is a notion used traditionally to measure the size of diffeomorphisms~[citeMallat and othermat].





\subsection{Stability of the Aggregation Operator}

Before stating formal results about stability, we discuss the characterization of the properties of the filters in the first layer of the regular CNN stage. To do so, we take into account the operators $\bbQ$  and $\bbA(\bbS)$, and we then characterize a subset algebraic filters in $\ccalC=\bigoplus_{i=1}^{\text{dim}(\ccalV_{0})}\mathbb{C}[t]$ using $\phi_{1}$. In particular, we attribute the properties of a set $\tilde{\ccalH}$ in the space of endomorphisms, to its pre-image $\ccalH$ in the algebra, this is

%
%
\begin{equation}
\ccalH
=
\left\lbrace
                \left.
                 h\in\bigoplus_{i=1}^{\text{dim}(\ccalV_{0})}\mathbb{C}[t]
                \right\vert
                               \quad \phi_{1}(h)\bbQ\bbA(\bbS)\in\tilde{\ccalH }                                   
\right\rbrace,
\end{equation} 
%
%

where the properties in $\tilde{\ccalH}$ are defined considering the operator $ \phi_{1}(h)\bbQ\bbA(\bbS)\in\tilde{\ccalH }$ a function of the shift operator(s) $\bbS$. We refer to $\ccalH$ as the set of algebraic filters with  properties given by $\tilde{\ccalH}$. It is worth pointing out that in this case there is a substantial difference with respect to the characterization of the filters when considering AlgNN where the filters are characterized as functions of the shift operators associated to the given representation.

Now we are ready to introduce two classes of filters that will be relevant for our stability discussion.



%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%% DEFINITION %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%

\begin{definition}\label{def_lipsintlips}

Let $(\ccalA,\ccalV,\rho)$ and $(\ccalC,\ccalU,\phi)$ be two algebraic signal models, where $\ccalA$ is generated by $g$. Let $\bbG(\bbS): \End{V}\to\End{U}$ with $\rho(g)=\bbS$. Then, we say that $p\in\ccalC$ is $\bbG(\bbS)$-induced Lipschitz with constant $L_{0}$ if the operator $\bbF(\bbS)=\phi(p)\bbG(\bbS)$ is $L_{0}$-Lipschitz in $\bbS$, this is

%
%
\begin{equation}
\left\Vert 
                \bbF(\bbS)-\bbF(\tilde{\bbS})
\right\Vert
                \leq
                     L_{0}
                             \left\Vert
                                            \bbS-\tilde{\bbS}
                             \right\Vert.
\end{equation}
%
%
%
Additionally, we say that $p\in\ccalC$ is $\bbG(\bbS)$-induced integral Lipschitz with constant $L_{1}$ if
%
%
%
\begin{equation}
\left\Vert  
                \bbD_{\bbF\vert\bbS}(\bbS) 
                                                           \left\lbrace
                                                                              \cdot\bbS
                                                           \right\rbrace
\right\Vert
                 \leq L_{1} 
                                \quad\forall\quad\bbS
\end{equation}
%
%
%
where $\bbD_{\bbF\vert\bbS}(\bbS)$ is the Fr\'echet derivative of $\bbF$ with respect to $\bbS$.
\end{definition}




Notice that Definition~(\ref{def_lipsintlips}), although the elements in $\ccalC$ are themselves functions of the shift operators associated to the signal model $(\ccalC,\ccalU,\phi)$, their properties are stated in terms of the shift operator of the signal model $(\ccalA,\ccalV,\rho)$. In what follows we denote the set of elemetns $p\in\ccalC$  that are $\bbG(\bbS)$-induced Lipschitz with constant $L_{0}$ as $\ccalC_{L_{0}}/\bbG(\bbS)$, while the set of $\bbG(\bbS)$-induced integral Lipschitz with constant $L_{1}$ as $\ccalC_{L_{1}}/\bbG(\bbS)$.

Now, we state the first result of stability showing how the changes in the composition of the aggregation operator, the mapping between the aggregation layer and the CNN, and filters in the first layer of the CNN are bounded by its Fr\'echet derivative.




%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%% THEOREM %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%

\begin{theorem}\label{theorem:HvsFrechet}

Let $(\ccalA,\ccalV,\rho)$ be the algebraic signal model associated to the aggregation layer of an Agg-AlgNN, $\Xi$, and $g$ the generator of $\ccalA$ with $\rho(g)=\bbS\in\text{End}(\ccalV)$. Let $\tilde{\rho}(g)=\tilde{\bbS}\in\text{End}(\mathcal{V})$ where the pair
$(\mathcal{V},\tilde{\rho})$ is a perturbed version of $(\mathcal{V},\rho)$ and $\tilde{\bbS}$ is related to $\bbS$ by the perturbation model in eqn.~(\ref{eqn_def_perturbation_model_20}).  Then, if $\bbF(\bbS)=\bbP\bbQ\bbA(\bbS)$, we have
%
%
%
\begin{equation}
\left\Vert
              \bbF(\bbS)\mathbf{x}-\bbF(\tilde{\bbS})\mathbf{x}
\right\Vert
                \leq 
                      \Vert\mathbf{x}\Vert
                                                      \left(
\left\Vert \bbD_{\bbF\vert\bbS}(\mathbf{S})\left\lbrace\mathbf{T}(\mathbf{S})\right\rbrace\right\Vert + \mathcal{O}\left(\Vert\mathbf{T}(\mathbf{S})\Vert^{2}
\right)
                                                        \right)
\label{eq:HSoptbound}
\end{equation}
%
%
%
where $\bbP$ is an operator acting on the first layer of the regular CNN of $\Xi$,  $\bbQ$ is the  operator that maps the information from the aggregation layer to the regular CNN stage of $\Xi$ and $\bbA(\bbS)$ is the aggregation operator. 

\end{theorem}
\begin{proof}
See Section~\ref{prooftheoremHvsFrechet}
\end{proof}


Theorem~\ref{theorem:HvsFrechet} states that the size of the changes in two operators associated to an Agg-AlgNN are bounded by the norm of the Fr\'echet derivative of the operator acting on the perturbation. In the following theorems, we make explicit how the norm of this operator acting on the perturbation is bounded.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%  THEOREM  %%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{theorem}\label{theorem:uppboundDH}

Let $(\ccalA,\ccalV,\rho)$ be the algebraic signal model associated to the aggregation layer of an Agg-AlgNN, $\Xi$, and let $\left( \bigoplus_{i=1}^{\text{dim}(\ccalV)}\mathbb{C}[t], \bigoplus_{i=1}^{\text{dim}(\ccalV)}\ccalR_{i}^{(1)}, \phi \right)$ the algebraic signal model in the first layer of the regular CNN of $\Xi$. Additionally, let $(\ccalA, \ccalV,\tilde{\rho})$ a perturbed version of $(\ccalA,\ccalV,\rho)$ associated with the perturbation model in eqn.~(\ref{eqn_perturbation_model_absolute_plus_relative}), $\bbQ$ the map between the aggregation layer and the CNN stage in $\Xi$ and $\bbA(\bbS)$ the aggregation operator. If $p\in\ccalC_{L_{0}}/\bbQ\bbA(\bbS)\cap\ccalC_{L_{1}}/\bbQ\bbA(\bbS)$ with $\ccalC=\bigoplus_{i=1}^{\text{dim}(\ccalV)}\mathbb{C}[t]$, we have that
%
%
%
\begin{equation}
\left\Vert 
             \bbD_{\bbF\vert\bbS}(\bbS)
                                                        \left\lbrace 
                                                        \bbT(\bbS)
                                                        \right\rbrace                  
\right\Vert
               \leq              
L_{0}\sup_{\bbS}\Vert\bbT(\bbS)\Vert +L_{1}\sup_{\bbS}\Vert D_{\bbT}(\bbS)\Vert
\label{eq:DHTS}
\end{equation}
%
%
%
where $\bbF(\bbS)=\bbP\bbQ\bbA(\bbS)$ and $\phi(p)=\bbP$.
 \end{theorem}
\begin{proof}See Section~\ref{prooftheoremuppboundDH}\end{proof}




From theorems~\ref{theorem:HvsFrechet} and~\ref{theorem:uppboundDH} we can state the notion of stability for algebraic filters in the following corollary.






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%  COROLLARY  %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{corollary}\label{corollary:DHboundsprcases}

Let $(\ccalA,\ccalV,\rho)$ be the algebraic signal model associated to the aggregation layer of an Agg-AlgNN, $\Xi$, and let $\left( \bigoplus_{i=1}^{\text{dim}(\ccalV)}\mathbb{C}[t], \bigoplus_{i=1}^{\text{dim}(\ccalV)}\ccalR_{i}^{(1)}, \phi \right)$ the algebraic signal model in the first layer of the regular CNN of $\Xi$. Additionally, let $(\ccalA, \ccalV,\tilde{\rho})$ a perturbed version of $(\ccalA,\ccalV,\rho)$ associated with the perturbation model in eqn.~(\ref{eqn_perturbation_model_absolute_plus_relative}), $\bbQ$ the map between the aggregation layer and the CNN stage in $\Xi$ and $\bbA(\bbS)$ the aggregation operator. Then, If $p\in\ccalC_{L_{0}}/\bbQ\bbA(\bbS)\cap\ccalC_{L_{1}}/\bbQ\bbA(\bbS)$ with $\ccalC=\bigoplus_{i=1}^{\text{dim}(\ccalV)}\mathbb{C}[t]$, the operator  $\bbF(\bbS)=\bbP\bbQ\bbA(\bbS)$ with $\phi(p)=\bbP$ is stable in the sense of definition~\ref{def:stabilityoperators1} with $C_{0}=L_{0}$ and $C_{1}=L_{1}$.

\end{corollary}
\begin{proof}
Replace (\ref{eq:DHTS}) from Theorem \ref{theorem:uppboundDH} into (\ref{eq:HSoptbound}) from Theorem \ref{theorem:HvsFrechet} and reorder terms.% to obtain the result in \eqref{eq:corollarTB}.
\end{proof}




















\blue{





%
%
\subsection{Stability of Algebraic Filters in Algebras with multiple geneators}

NOTE: In this section I will extend the analysis to cases where $\ccalA$ has multiple generators

%
%The stability results presented in previous subsection can be extended naturally to operators associated to representations of algebras with multiple generators. Before doing so, we extend the notions used to characterize subsets of algebras. If $\mathcal{A}$ is the algebra generated by $\{g_{i}\}_{i=1}^{m}$ and $g_{i}g_{j}=g_{j}g_{i}$ for all $i,j$ with coefficients in $\mathbb{R}$, we use the isomorphism $\iota:\mathcal{A}\rightarrow\mathcal{A}_{\mathbb{C}}$ given by $\iota(g_{i})=\lambda_{i}\in\mathbb{C}$. Then, we can use $\iota\left(p_{\mathcal{A}}(g_{1},\ldots,g_{m})\right)=p(\boldsymbol{\lambda})$ where $\boldsymbol{\lambda}=(\lambda_{1},\ldots,\lambda_{m})\in\mathbb{C}^{m}$ to characterize elements in $\mathcal{A}$. Therefore, stating conditions on $p(\boldsymbol{\lambda})$ we can define subsets of $\mathcal{A}$ via $\iota^{-1}$. In the following definition we extend the concepts presented in previous subsection.
%
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% DEFINITION %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%\begin{definition}
%Let $p:\mathbb{C}^{m}\rightarrow\mathbb{C}$ be  a multivariate function. Then, it is said that $p$ is Lipschitz if there exists $L_{0}>0$ such that
%\begin{equation}
%\vert p(\boldsymbol{\lam})-p(\boldsymbol{\mu})\vert\leq L_{0}\Vert\boldsymbol{\lam}-\boldsymbol{\mu}\Vert
%\end{equation}
%for all $\boldsymbol{\lambda},\boldsymbol{\mu}\in\mathbb{C}^{m}$. Additionally, it is said that $p(\boldsymbol{\lambda})$ is Lipschitz integral if there exists $L_{1}>0$ such that
%%
%\begin{equation}
%\left\vert \lambda_{i}\frac{\partial p(\boldsymbol{\lambda})}{\partial \lambda_{i}}\right\vert\leq L_{1}\quad\forall~i\in\{1,\ldots m \},
%\end{equation}
%%
%where $\boldsymbol{\lambda}=(\lambda_{1},\ldots,\lambda_{m})$.
%\end{definition}
%%
%With this notion at hand, we are ready to  extend the stability theorems.
%
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% THEOREM %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%\begin{theorem}\label{theorem:HvsFrechetmultgen}
%Let $\mathcal{A}$ be an algebra generated by $\{g_{i}\}_{i=1}^{m}$ and let $(\mathcal{M},\rho)$ be a representation of $\mathcal{A}$ with $\rho(g_{i})=\bbS_{i}\in\text{End}(\mathcal{M})$ for all $i$. Let $\tilde{\rho}(g_{i})=\tilde{\bbS}_{i}\in\text{End}(\mathcal{M})$ where the pair
%$(\mathcal{M},\tilde{\rho})$ is a perturbed version of $(\mathcal{M},\rho)$ and $\tilde{\bbS}_{i}$ is related to $\bbS_{i}$ by the perturbation model in eqn.~(\ref{eqn_def_perturbation_model_20}). Then, for any $p_{\mathcal{A}}\in\mathcal{A}$ we have
%%
%\begin{equation}
%\left\Vert p(\bbS)\mathbf{x}-p(\tilde{\bbS})\mathbf{x}\right\Vert\leq 
%\Vert\mathbf{x}\Vert\sum_{i=1}^{m}\left(\left\Vert D_{p\vert\mathbf{S}_{i}}(\mathbf{S})\mathbf{T}(\mathbf{S}_{i})\right\Vert+\mathcal{O}\left(\Vert\mathbf{T}(\mathbf{S}_{i})\Vert^{2}\right)\right)
%\label{eq:HSoptboundmultgen}
%\end{equation}
%%
%where $D_{p\vert\mathbf{S}_{i}}(\mathbf{S})$ is the partial Fr\'echet derivative of $p$ on $\mathbf{S}_{i}$.
%\end{theorem}
%\begin{proof}
%See Section~\ref{prooftheoremHvsFrechet}
%\end{proof}
%%
%Notice that in eqn.~(\ref{eq:HSoptboundmultgen}) we naturally add the contribution associated to each generator. Therefore, to guarantee stability we must have stability in each generator. Now, we show how the Fr\'echet derivative of $\mathbf{T}(\mathbf{S})$ is involved in the stability properties when considering multiple generators.
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% THEOREM %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\begin{theorem}\label{theorem:uppboundDHmultg}
%Let $\mathcal{A}$ be an algebra with $m$ generators $\{g_{i}\}_{i=1}^{m}$ and $g_{i}g_{j}=g_{j}g_{i}$ for all $i,j\in\{1,\ldots m\}$. Let $(\mathcal{M},\rho)$ be a finite or countable infinite dimensional representation of $\mathcal{A}$ and $(\mathcal{M},\tilde{\rho})$ a perturbed version of $(\mathcal{M},\rho)$ related by the perturbation model in eqn.~(\ref{eqn_perturbation_model_absolute_plus_relative}).  Then, if $p_{\mathcal{A}}\in\mathcal{A}_{L_{0}}\cap\mathcal{A}_{L_{1}}$ it holds that
%%
%\begin{multline}
%\left\Vert D_{p\vert\mathbf{S}_{i}}(\mathbf{S})\bbT(\bbS_{i})\right\Vert
%\\
%\leq (1+\delta)
%\left(
%L_{0}\sup_{\bbS_{i}\in\mathcal{S}}\Vert\bbT(\bbS_{i})\Vert +L_{1}\sup_{\bbS_{i}\in\mathcal{S}}\Vert D_{\bbT}(\bbS_{i})\Vert\right)
%\label{eq:DHTSmultg}
%\end{multline}
% \end{theorem}
% \begin{proof}See Section~\ref{prooftheorem:uppboundDH}\end{proof}
% %
% It is important to remark that the upper bound in eqn.~(\ref{eq:DHTSmultg}) is defined by the largest perturbation in a given generator although the constants associated are determined completely by the properties of the filters.
% 
%From theorems~\ref{theorem:HvsFrechetmultgen} and~\ref{theorem:uppboundDHmultg} we can state the stability results for filters in algebras with multiple generators in the following corollary.
%%
%\begin{corollary}\label{corollary:stabmultgenfilt}
%Let $\mathcal{A}$ be an algebra with generators $\{ g_{i}\}_{i=1}^{m}$ and $g_{i}g_{j}=g_{j}g_{i}$ for all $i,j$. Let $(\mathcal{M},\rho)$ be a finite or countable infinite dimensional representation of $\mathcal{A}$ and $(\mathcal{M},\tilde{\rho})$ be a perturbed version of $(\mathcal{M},\rho)$ related by the perturbation model in eqn.~(\ref{eqn_perturbation_model_absolute_plus_relative}). Then, if $p_{\mathcal{A}}\in\mathcal{A}_{L_{0}}\cup\mathcal{A}_{L_{1}}$ the operator $p(\mathbf{S})$ is stable in the sense of definition~\ref{def:stabilityoperators1} with $C_{0}=m(1+\delta)L_{0}$ and $C_{1}=m(1+\delta)L_{1}$.
%%%
%%we have
%%%
%%\begin{multline}
%%\frac{\left\Vert p(\bbS)\mathbf{x}-p(\tilde{\bbS})\mathbf{x}\right\Vert}{\Vert\mathbf{x}\Vert}
%%\leq 
%%\sum_{i=1}^{m}\left[ (1+\delta)
%%\left(
%%L_{0}\sup_{\bbS_{i}\in\mathcal{S}}\Vert\bbT(\bbS_{i})\Vert\right.\right.
%%\\
%%\left.\left. +L_{1}\sup_{\bbS_{i}\in\mathcal{S}}\Vert D_{\bbT}(\bbS_{i})\Vert\right)+\mathcal{O}\left(\Vert\mathbf{T}(\mathbf{S}_{i})\Vert^{2}\right)\right]
%%\end{multline}
%%for all $\mathbf{x}\neq\mathbf{0}$.
%%
%\end{corollary}
%\begin{proof} Replacing eqn.~(\ref{eq:DHTSmultg}) from theorem~\ref{theorem:uppboundDHmultg} into eqn.~(\ref{eq:HSoptboundmultgen}) from theorem~\ref{theorem:HvsFrechetmultgen} and organazing the terms.\end{proof}

}








\subsection{Stability of  Aggregation Algebraic Neural Networks}

In this section we extend the stability results presented above to operators that represent general Agg-AlgNN with an arbitrary number of layers. Given an Agg-AlgNN, 
%
$\Xi=\left\lbrace
                        \left.
                               (\ccalA,\ccalV,\rho)
                        \right\vert
                                        \text{\texttt{CNN}}(L,F_{\ell})       
\right\rbrace$,
%
we say its perturbed version is 
%
$\tilde{\Xi}=\left\lbrace
                        \left.
                               (\ccalA,\ccalV,\tilde{\rho})
                        \right\vert
                                        \text{\texttt{CNN}}(L,F_{\ell})       
\right\rbrace$,
%
where $(\ccalA,\ccalV,\tilde{\rho})$ is a perturbed version of $ (\ccalA,\ccalV,\rho)$ in the sense of definition~\ref{def:perturbmodel}. We start considering results when the algebra $\ccalA$ has one generator and for the sake of simplicity that the number of features per layer is $F_{\ell}=1$. Notice however, that the theorems can be easily extended to cases where several features are considered. 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%% THEOREM STABILITY ALGNN 1%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{theorem}\label{theorem:stabilityAlgNN0}

Let
%
$\Xi=\left\lbrace
                        \left.
                               (\ccalA,\ccalV,\rho)
                        \right\vert
                                        \text{\texttt{CNN}}(L,1)       
\right\rbrace$,
%
be an Agg-AlgNN and
%
$\tilde{\Xi}=\left\lbrace
                        \left.
                               (\ccalA,\ccalV,\tilde{\rho})
                        \right\vert
                                        \text{\texttt{CNN}}(L,F_{\ell})       
\right\rbrace$,
%
the perturbed version of $\tilde{\Xi}$ by means of the perturbation model in eqn.~(\ref{eqn_perturbation_model_absolute_plus_relative}). Then, if $\Phi_{\Xi}$ and 
$\Phi_{\tilde{\Xi}}$ represent the mapping operators associated to $\Xi$ and $\tilde{\Xi}$ we have
%
%
%
\begin{multline}\label{eq:theoremstabilityAlgNN0}
\left\Vert
                 \Phi_{\Xi}(\bbx) -  \Phi_{\tilde{\Xi}}(\bbx)
\right\Vert
                \leq
\\                
                       \left(
                               \prod_{\ell=1}^{L}{C}_{\ell}
                       \right) 
                       \left(
                               \prod_{\ell=2}^{L}{B}_{\ell}
                       \right)
                                \left(
                                         L_{0}\sup_{\bbS} \Vert \bbT(\bbS) \Vert
                                         +
                                         L_{1}\sup_{\bbS} \Vert  \bbD_{\bbT}(\bbS) \Vert
                                \right)
                                         \Vert \bbx \Vert
\end{multline}
%
%
%
where $C_{\ell}$ is the Lipschitz constant of $\sigma_{\ell}$, $\Vert \bbH_{\ell}\Vert\leq B_{\ell}$.
\end{theorem}
\begin{proof}See Section~\ref{prooftheorem:stabilityAlgNN0}\end{proof}




\subsection{Implications for Aggregation GNNs}

The stability results for aggregation GNNs are obtained as a direct byproduct of the results derived before. In this section we put those results in the concrete scenario of GNNs, using matrix and making more specific the meaning of Definition~\ref{def_lipsintlips} when considering the aggregation operator in GNNs.


\blue{
--- NOTE: Here make a remark about the implications for  graph aggregation neural networks
}


\blue{
\subsection{Stability: Aggregation vs Section AlgNNs}
--- NOTE: Here maybe we can discuss the comparison of the stability bounds with respect to the ones we obtain for selection neural networks. It might be more difficult to ensure conditions in the aggregation... 
}












